Solving realistic security-constrained optimal power flow problems

We present a decomposition approach for obtaining good feasible solutions for the security-constrained alternating-current optimal power flow (SCACOPF) problem at an industrial scale and under real-world time and computational limits. The approach aims at complementing the existing body of literature on bounding the problem via convex relaxations. It was designed for the participation in ARPA-E's Grid Optimization (GO) Competition Challenge 1. The challenge focused on a near-real-time version of the SCACOPF problem where a base case operating point is optimized taking into account possible single-element contingencies, after which the system adapts its operating point following the response of automatic frequency drop controllers and voltage regulators. Our solution approach for this problem relies on state-of-the-art nonlinear programming algorithms and employs nonconvex relaxations for complementarity constraints, a specialized two-stage decomposition technique with sparse approximations of recourse terms, and contingency ranking and pre-screening. The paper also outlines the salient features of our implementation, such as fast model functions and derivatives evaluation, warm-starting strategies, and asynchronous parallelism. We discuss the results of the independent benchmark of our approach done by ARPA-E's GO team in Challenge 1, which found that our methodology consistently produces high quality solutions across a wide range of network sizes and difficulty. Finally, we conclude by outlining potential extensions and improvements of our methodology.

==> electronic_companion.tex <==
%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ECSwitch

%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Proofs of Statements}

A general heading for the whole e-companion should be provided here as in the example above this paragraph.

\section{Proof of Theorem \ref{marg-butt-th}.}

To avoid confusion, theorems that we repeat for readers' convenience
will have the same appearance as when they were mentioned for the first
time. However, here they should be coded by \verb+repeattheorem+ instead
of \verb+theorem+ to keep labels/pointers uniquely resolvable. Other predefined theorem-like
environments work similarly if they need to be repeated in what becomes the \mbox{e-companion.}


\begin{repeattheorem}[Theorem 1.]
%\label{marg-butt-th}
In a reverse dictionary, $(\mbox{\bi marg}\succ\mbox{\bi butt\/}\; \land\;  
\mbox{\bi arine}\succ\mbox{\bi er})$.
Moreover, continuous reading of a compact subset of the dictionary
attains the minimum of patience at the moment of giving up.
\end{repeattheorem}

\subsection{Preparatory Material}

\begin{lemma}
\label{aux-lem1}
In a reverse dictionary, $\mbox{\bi g}\succ\mbox{\bi t\/}$.
\end{lemma}

\begin{lemma}
\label{aux-lem2}
In a reverse dictionary, $\mbox{\bi e}\succ\mbox{\bi r\/}$.
\end{lemma}

\proof{Proof of Lemmas \ref{aux-lem1} and \ref{aux-lem2}.} See the alphabet and the tebahpla.\Halmos
\endproof

\begin{remark} 
Note that the title of the proof should be keyed
explicitly in each case. Authors can hardly agree on what would be the
default proof title, so there is no default. Even \verb+\proof{Proof.}+ should be keyed out. 
\end{remark}


\subsection{Proof of the Main Result}

\proof{Proof of Theorem 1.} The first statement is a conseqence of
Lemmas~\ref{aux-lem1} and \ref{aux-lem2}. The rest relies on the fact that the continuous
image of a compact set into the reals is a closed interval, thus having
a minimum point.\Halmos 
\endproof

%\begin{figure}[t]
%\begin{center}
%\includegraphics[height=1.5in]{Sample-Figure}
%\caption{Production Possibilities Frontier Again.} \label{ECfrontier}
%\end{center}
%\end{figure}




% Appendix here
% Options are (1) APPENDIX (with or without general title) or
%             (2) APPENDICES (if it has more than one unrelated sections)
% Outcomment the appropriate case if necessary
%
% \begin{APPENDIX}{<Title of the Appendix>}
% \end{APPENDIX}
%
%   or
%
% \begin{APPENDICES}
% \section{<Title of Section A>}
% \section{<Title of Section B>}
% etc
% \end{APPENDICES}


% Acknowledgments here
\ACKNOWLEDGMENT{The authors gratefully acknowledge the existence of
the Journal of Irreproducible Results and the support of the Society
for the Preservation of Inane Research.}


% References here (outcomment the appropriate case)

% CASE 1: BiBTeX used to constantly update the references
%   (while the paper is being written).
%\bibliographystyle{informs2014} % outcomment this and next line in Case 1
%\bibliography{<your bib file(s)>} % if more than one, comma separated

% CASE 2: BiBTeX used to generate mypaper.bbl (to be further fine tuned)
%\input{mypaper.bbl} % outcomment this line in Case 2

%If you don't use BiBTex, you can manually itemize references as shown below.

\begin{thebibliography}{}

\bibitem[{Feldman and Schwan(1990)}]{fs}
Feldman D, Schwan K (1990) {\it Who Put the Butter in Butterfly
and Other Fearless Investigations into Our Illogical Language}
(HarperPerennial, New York).

\bibitem[{Fontecha et~al.(2006)}]{fo}
Fontecha J, Mayo I, Toledano G, Juarez M (2006)
Triacylglycerol composition  of projected designation
of origin cheeses during ripening. {\it J. Dairy Sci.} 89:882--887.

\bibitem[{Geisel(1984)}]{g}
Geisel TS (1984) {\it The Butter Battle Book\/} (Random House, New York).

\bibitem[{Hodson et~al.(2001)}]{h}
Hodson L, Skeaff CM, Chisholm W-AH (2001) The effect of
replacing dietary saturated fat with polyunsaturated or
monounsaturated fat on plasma lipids in free-living young adults.
{\it Eur. J. Clinical Nutrition} 55(10):908--915.

\bibitem[{Tholstrup et al.(2006)}]{trbn} 
Tholstrup T, Raff M, Basu S, Nonboe P, Sejrsen K, Staarup EM (2006) 
Effects of butter and mono\-un\-saturated fatty acids
into lipid classes, plasma C-reactive protein, oxidative stress,
hemostatic variables, and insulin in healthy young men. {\it Amer. J.
Clinical Nutrition} 83:237--243.
\bibitem[{Torbica et al.(2006)}]{tjp}
Torbica A, Jovanovic O, Pajin B (2006) The advantages of solid
fat content determination in cocoa butter and cocoa butter
equivalents by the Karlshamns method. {\it Eur. Food Res. Techn.} 222:385--391.

\end{thebibliography}

